Evaluating few shot and Contrastive learning Methods for Code Clone Detection

Context: Code Clone Detection (CCD) is a software engineering task that is used for plagiarism detection, code search, and code comprehension. Recently, deep learning-based models have achieved an F1 score (a metric used to assess classifiers) of $\sim$95\% on the CodeXGLUE benchmark. These models require many training data, mainly fine-tuned on Java or C++ datasets. However, no previous study evaluates the generalizability of these models where a limited amount of annotated data is available. Objective: The main objective of this research is to assess the ability of the CCD models as well as few shot learning algorithms for unseen programming problems and new languages (i.e., the model is not trained on these problems/languages). Method: We assess the generalizability of the state of the art models for CCD in few shot settings (i.e., only a few samples are available for fine-tuning) by setting three scenarios: i) unseen problems, ii) unseen languages, iii) combination of new languages and new problems. We choose three datasets of BigCloneBench, POJ-104, and CodeNet and Java, C++, and Ruby languages. Then, we employ Model Agnostic Meta-learning (MAML), where the model learns a meta-learner capable of extracting transferable knowledge from the train set; so that the model can be fine-tuned using a few samples. Finally, we combine contrastive learning with MAML to further study whether it can improve the results of MAML.

==> NEW_STRUCTURE.tex <==
\section{Introduction} \label{intro}


Code Clone Detection (CCD) refers to finding functionally similar code fragments (pairs). CCD can cause buggy code to propagate through the whole project \cite{shobha2021code,roy2018benchmarks,bellon2007comparison} and is necessary to develop and maintain source code \cite{LEI2022111141}. 
It is an important task for many software engineering applications including finding library candidates, code comprehension, finding harmful software, and plagiarism detection \cite{ain2019systematic}. 
There are a lot of studies that develop models to detect code clones \cite{wang2021syncobert,wang2020detecting,wang-etal-2021-codet5}. 

Although the state-of-the-art models achieve an {F1-Score} (a score used for classification task) of approximately $96$ percent on the BigCloneBench data {\cite{wang2021syncobert}} and MAP@R score (a metric used for information retrieval based CCD task) of $88$ percent on POJ-104 {\cite{wang2021syncobert}} --the widely used benchmark datasets for CCD-- the ability of the current state-of-the-art models for CCD to be generalized to \textit{unseen programming languages} and \textit{unseen programming problems} is rarely studied \cite{sonnekalb2022generalizability, liu2021can}. 
\textcolor{teal}{In other words, the ability of the model to detect code clones for a language that it has not been trained on (i.e., unseen programming languages), or the ability of the model to detect code clones of which their functionality have never been observed in the training data (i.e., unseen programming problems), which is one of the main aspects of our study. }
In the rest of the paper, we will refer to `programming languages' as `languages' and `programming problems' as `problems' for simplicity.

% Second, training CCD models requires a lot of training data, which is costly to build.
Lei et al. report that $84$ percent of CCD studies mainly use BigCloneBench which has over six million code pairs \cite{wang2020detecting} and POJ-104 which has 52,000 code samples \cite{mou2016convolutional,LEI2022111141}. 
However, many other programming languages have restricted labeled data, and generating annotated CCD data for these languages requires extensive time and effort {\cite{zhang2022graph}}.
Given the restricted labeled data for other programming languages and the costs of curating new datasets and training the models on new datasets, there is a need for models that perform well where there is little training data available, and are generalizable to new problems and new programming languages. 


Hence, in this study, we first evaluate the ability of the models in three scenarios: i) the model is applied on new problem sets, ii) the model has not seen the programming language during training, and iii) a combination of both. 
We conduct our study in a more rigorous way and evaluate the models in a few-shot setting, i.e., cases where \textbf{only a few examples are available for training the models} instead of thousands or millions of samples.




% , addressing the costs associated with curating high quality datasets and retraining the models. 
We then investigate a few-shot learning technique using an algorithm named 
Model-Agnostic Meta-Learning (MAML) \cite{finn2017model}, which aims to learn parameters that are sensitive to change and assess whether it can increase the performance of the models in a few-shot setting.
Few-shot learning is a specific approach developed for transferring the knowledge that a model has learned by training on a high resource domain/task (i.e., there exists a lot of labeled data) to a low resource domain/task (i.e., when limited labeled data is available) \cite{zhang2022graph}.
\textcolor{purple}{MAML is chosen because it is a well-established method in few-shot learning \cite{walsh2022automated,ye2021train,finn2017model}. Additionally, it can be applied to any gradient descent approach, making it a convenient method for training a meta-learner on top of the baselines experimented in our study.}

Furthermore, we integrate contrastive learning with MAML to assess if we can improve the results of the models. 
Contrastive learning is a self-supervised learning approach that aims to create a similar representation for positive samples and a different embedding for negative ones. This method does not need any labeled data and trains an objective that pulls positive samples together and pushes negative instances apart. 
As code clones should also have similar representation, we hypothesize that using contrastive learning is beneficial for few-shot learning of CCD in the above three mentioned scenarios. 
\textcolor{teal}{This study is providing the results of our previously accepted Registered Report in The 2022 Mining Software Repositories Conference (MSR)  \footnote{https://conf.researchr.org/track/msr-2022/msr-2022-registered-reports?#event-overview}.}

It is worth noting that recently, a new trend has been started in code understanding studies toward using general-purpose generative models for solving few-shot learning problems. In this line of research, Few-Shot, Pre-Trained Language Models (FSLMs) like GPT-3 \cite{brown2020language} and CodeX \cite{chen2021evaluating} are used for various programming problems, such as code mutation, test case generation, and fabricating oracles from natural language documentation \cite{bareiss2022code}. 
As a result, these studies have shifted toward designing a prompt that encourages the FSLM to generate a specific code fragment. This code fragment is employed to address a code understanding task. For instance, in \cite{bareiss2022code}, prompt engineering and FSMLs are utilized to address code mutation, oracle generation from natural language documentation, and making unit tests.
Moreover, Pearce et al.\cite{pearce2022examining} study the capability of commercial large language models to solve security bugs in the code. 
It is worth noting that FSLM models are primarily used for generative tasks and have not been applied to classification tasks such as code clone detection. Though we do not use them here, we investigate the few-shot learning approach, which similar to FSLM, emphasizes on availability of only a few labeled data for downstream tasks.


In our study, we seek the answer to the following research questions: 

\textbf {RQ1: What is the performance of the current state-of-the-art models for code clone detection when they are fine-tuned on a few examples of the downstream task?} 

\textit{Here, we empirically study to what extent the current CCD models perform when trained on a few samples of a new downstream language or problem set. So, we evaluate these models on languages and problems that the model has not seen during the fine-tuning phase. Our results show that the current state-of-the-art models for CCD are susceptible to unseen problems and unseen languages.}


\textbf{RQ2: What is the performance of a few-shot learning method for code clone detection?}

\textit{In this RQ, we evaluate the performance of the models when a few-shot learning technique is applied. Our findings indicate that using MAML can improve the performance of the baselines by $\sim20$ percent for unseen problems in C++ and Ruby. Yet, using MAML has a negligible effect on the accuracy of the CCD model for unseen languages. }

\textbf{RQ3: Can we improve the performance of the few-shot learning models by using a contrastive learning model as the baseline for training? }

\textit{As the representation of source code with contrastive learning objective has shown to be useful for code clone detection \cite{oord2018representation,wang2021syncobert,jain-etal-2021-contrastive}, it is used with the few-shot algorithm in RQ3. The results show that using ContraCode, which possesses a contrastive objective, does not improve the accuracy of MAML.}


 

The contributions of this work are as follows: 

\begin{itemize}
    \item Evaluating code clone detection models in the context of few-shot learning, for both unseen problems and unseen programming languages.
    \item Integrating contrastive learning with a few-shot algorithm. 
\end{itemize}
 
 
The results can shed light on the generalizability of clone detection models for languages and programming problems for which the number of available labeled data is limited. 


\textcolor{blue}{\textbf{Deviations from the Registered Report.} First, the POJ-104 and BigCloneBench datasets are not used and we ran all experiments on CodeNet dataset. 
The rationale was that the number of problems (functionalities) are limited in BigCloneBench. Also, for the third scenario, we needed to have the solutions for one problem set from different languages, which was not available in these datasets. Thefore, we considered our extracted dataset from CodeNet in all experiments.
Second, in our report, we initially intended to compare the results against BERT, RoBERTa, CodeBERT, TBCCD, CDLH, and ContraCode. However, in our results presented here we did not use BERT and CDLH models. The reason is that in many Natural Language Processing and Software Engineering tasks, RoBERTa performs better than BERT. Also, CDLH does not have public scripts, and thus is eliminated from our experiments. Another deviation is that in the second scenario, unseen languages, we intended to have only C++ and Ruby as unseen languages. However, we extended our experiments and also studied the cases where the model is trained on C++ and is tested on Java (i.e., also considering Java as the unseen language). Finally, we restricted the number of experiments compared to what we mentioned in the RR. Training MAML is computationally expensive. As a result, when we conducted the experiments and observed the results, we decided to eliminate some experiments, as we expected similar results would be obtained for the retrieval-based CCD. First, we conducted scenarios I and II (unseen problems and unseen languages) for binary CCD. In the third scenario, we conducted the binary CCD for all models and we eliminated RoBERTa, as it had slightly lower scores than CodeBERT in the previous two scenarios. However, for the retrieval-based CCD, we decided to eliminate most experiments due to the above-mentioned reasons. Thus, we only conducted the retrieval-based CCD for the third scenario.}


The rest of this report is organized as follows. 
First, we provide the related works and the required background in Sections \ref{sec:lr} and \ref{sec:background}. We discuss the methodology in Section \ref{sec:method}. 
For each of the studied scenarios, we dedicate a separate section including the approach, results, and discussions for that scenario. The details of our experiments for unseen problems are provided in Section \ref{sec:scenario-i}. The unseen programming languages are discussed in Section \ref{sec:scenario-ii} and Section \ref{sec:scenario-iii} is dedicated to the third scenario (i.e., unseen problems and programming languages). 
The implications are discussed in Section \ref{sec:implications}, which is followed by threats to validity in Section \ref{sec:threats}. Finally, we conclude the paper in Section \ref{sec:conclusion}.




\section{Literature Review} \label{sec:lr}

One of the early approaches to code clone detection was based on lexical similarity, where code snippets are compared based on their syntax and structure \cite{ain2019systematic}. However, lexical similarity alone is not always sufficient to identify code clones, as the same functionality can be implemented using different syntax and structure \cite{LEI2022111141}. To overcome this limitation later approaches incorporated semantic similarity into the code clone detection process, where the functional equivalence of code snippets is considered \cite{ye2020misim,feng-etal-2020-codebert,yu2019neural}.
Another approach to code clone detection is based on program analysis, where code is analyzed at the Abstract Syntax Tree (AST) level, and code clones are identified based on the similarity of their ASTs \cite{yu2019neural}. 
% This approach is more robust than lexical similarity-based approaches, \textcolor{red}{as it considers the structural equivalence of code snippets in addition to the lexical similarity.}

More recently, deep learning-based approaches have been proposed for code clone detection. These approaches use various algorithms, such as clustering and classification, to identify code clones \cite{yuan2022java}. Deep learning-based approaches are shown to be more accurate than other approaches, as they can learn from large amounts of code clone data and incorporate structural and lexical as well as semantic similarity in the code clone detection process \cite{zhang2023challenging,feng-etal-2020-codebert,wi2022hiddencpg}. 
CDLH \cite{wei2017supervised} is one such approach that employs a Long Short Term Memory (LSTM) model  based on abstract syntax trees to represent code fragments. ASTNN \cite{zhang2019novel} is another method that uses ASTs to encode the subtrees of a tree and employs a Recurrent Neural Network (RNN) to produce embeddings of code snippets. FA-ASTGMN \cite{wang2020detecting} uses Graph Neural Networks (GNNs) to encode the control and data flow of code snippets through ASTs. 
TBCCD \cite{yu2019neural} is a study proposing a tree-based convolution method and a Siamese network to encode the structure and semantics of code fragments, which has demonstrated effectiveness in detecting code clones. 

More recently, pre-trained language models are used for code clone detection. 
In recent years, pre-trained models have gained significant attention in the field of code understanding including code clone detection due to their ability to leverage large amounts of code data and generalize well to new datasets. 
This paradigm's fundamental principle is to initially train a model on broad, general-purpose datasets using self-supervised tasks such as masking tokens in training data and guiding the model to predict the masked tokens. 
Following this, the model is further trained on smaller and more specific datasets tailored to support a particular task \cite{wang2022bridging}. 
As a result, several pre-trained models, including CodeBERT \cite{feng-etal-2020-codebert}, RoBERTa \cite{liu2019roberta}, GraphCodeBERT \cite{GuoRLFT0ZDSFTDC21}, PLBART \cite{ahmad-etal-2021-unified}, CodeT5 \cite{wang-etal-2021-codet5}, and DOBF \cite{lachaux2021dobf} have demonstrated successful performance in detecting code clones. 
% A more recent approach, DOBF \cite{lachaux2021dobf}, introduces a novel objective that pre-trains a model, surpassing other pre-trained models such as CodeBERT and GraphCodeBERT in various downstream tasks, including code clone detection. 

While existing pre-trained models have demonstrated success in code clone detection tasks, they have millions of parameters, potentially leading to overfitting when applied to specialized small datasets.
Numerous studies indicate that pre-trained models perform poorly when tested on data that differs significantly from the training set \cite{quiring2019misleading,yefet2020adversarial}. 
To remedy this issue, several studies propose data augmentation techniques to address the vulnerability of pre-trained models for out-of-domain test data in code-related tasks \cite{zhang2020generating,rabin2021generalizability,wang2022bridging}. For example, Wang et al. \cite{wang2022bridging} proposed a data augmentation approach that incorporates an easy-to-hard sequence of augmented data into the model. \textit{While these studies aim to address the same problem as the current research, they do not extend to domains with extremely limited training data, requiring the adaptation of the model to only a few training samples.} 

\textcolor{blue}{Sonnekalb et al. \cite{sonnekalb2022generalizability} empirically studied the performance of CodeBERT on various versions of BigCloneBench. In their study, they proposed curating a dataset with different functionalities for training and testing. They concluded that the accuracy of CodeBERT dropped from 94.40\% to 48.97\% simply by testing the model on a different version of the same dataset.
Similarly, Liu et al. \cite{liu2021can} investigated the generalizability of TBCCD \cite{yu2019neural} and ASTNN \cite{zhang2019novel}, two major models for code clone detection, for unseen functionalities. In their research, they used OJClone as the benchmark, which consists of 104 functionalities (problems). They organized the functionalities into 7 groups, following an approach similar to that used in TBCCD. They discovered that the performance of these models declined by more than 50\% for some unseen functionalities. They attributed the poor performance to three main reasons: {Training Data Diversity}, {Unseen Vocabulary}, and Locality.
\textit{The primary distinction between their work and our study lies in our focus on few-shot learning. Specifically, we aim to fine-tune models with only a few instances of the downstream tasks. Additionally, we investigate the performance of the models for unseen languages, which are not done in these works.}}



Cross-Language Code Clone Detection (CLCCD) is a closely related research area to the current research that has gained attention in recent years. CLCCD focuses on detecting code clones across different programming languages, which is a challenging task since code written in different languages may have varying syntax and structure, even if they serve the same purpose. To address this challenge, researchers have proposed models that can detect code clones across different programming languages \cite{tao2022c4,nafi2019clcdsa,ankali2021detection}. The difference between CLCCD and our research on unseen languages is that CLCCD studies detect clones in various languages, but the models are trained and tested on a \textit{combined} set of programming languages. Therefore, if we intend to use the same model to detect clones in a different programming language that was not included in the training set, we must create a new dataset from scratch. This limits the model's ability to generalize to \textit{unseen} programming languages\footnote{Thus, we do not focus on CLCCD and our focus is only on CCD in this work. It is worth mentioning that applying the same techniques can be interesting to assess the ability of the CLCCD models, but this is out of the scope of our work, due to the high number of required experiments and limited computational resources.}. 
\textcolor{purple}{It is worth noting that the studies that address CLCCD are much fewer than the ones that investigate code clone detection in one programming language. Moreover, most of these CLCCD methods focus solely on Java, Python, and C\# and overlook other low-resource languages like Ruby \cite{nafi2019clcdsa,perez2019cross}. }
% It is worth noting that from all code clone detection methods, only 10 percent develop models for CLCCD, but they are also conducted on Java, Python, and C\#.

%{The recent deep learning pre-trained language models such as GraphCodeBERT {\cite{guo2020graphcodebert}}, CodeBERT \cite{feng2020codebert}, and RoBERTa \cite{liu2019roberta} are among the studies that achieve the state-of-the-arts results for CCD. However, they have not studied the performance of the models for new languages and new problem sets. They fine-tune their model on BigCloneBench or POJ-104 which are highly resourced languages, and the language of the dataset was seen during their pre-training. Therefore, the ability of these models in the presence of little CCD training data is unknown.}


% Previous studies neglected the generalizability of CCD models.  If one wants to use an existing model for a language to detect code clones in a new language, the model should be retrained again using a large number of training data in the new language. However, preparing such data is expensive and time-consuming.  
% There are many use cases in which the model needs to be generalized. Data science, where developers are looking for the solution to the same problem in different languages \cite{mathew2021cross,nafi2019clcdsa}, or cross-platform software development, where the companies make the same application for different platforms are among the applications of a generalizable model \cite{nafi2019clcdsa}. 

% Apart from the vulnerability of CCD models to be generalized to new languages, if the code fragments are from different problem sets, the ability of the models to detect them is shown to be downgraded significantly \cite{yu2019neural}.
% For example, Yu et al. \cite{yu2019neural} present TBCCD for code clone detection, which achieves {an F1-Score of 99 percent on a binary classification version of POJ-104 data}, but they show that their model is susceptible in the face of unseen problems. The performance of their model drops to {49 percent on average} when trained and tested on disjoint sets of problems (i.e. tested on unseen problems), but the authors do not provide any solutions. 

% Moreover, while there exist many submissions for some programming problems, which can be used to learn their semantics for CCD, there are problems for which only a few solutions exist, making the CCD data for training the model in that domain hard. %\textcolor{red}{TODO: any example for this? I can mention Graph homomorphism and Clique cover problems. However, I don't have any reference for this claim.}
% Note that the second scenario is closely related to CLCCD, where the model is only trained on one language and is tested on another language, but different in the sense that the current CLCCD models are trained on a combination of the languages that require clone detection



% Few-shot learning models are widely studied in computer vision \cite{vinyals2016matching,snell2017prototypical,sung2018learning} and there are few works conducted on using few-shot learning for natural language processing \cite{yin2020universal,bansal2019learning}. However, \textbf{no previous study has been conducted on applying few-shot learning algorithms for code clone detection.}


\textbf{Differences with the existing research:} 
The study of code clone detection models in a few-shot setting that we address in our work here is new. Though previous works assessed the performance of their model for different problem sets \cite{yu2019neural} or tackle the cross-lingual code clone detection \cite{tao2022c4,nafi2019clcdsa,ankali2021detection}, the current research differs from our work from a few perspectives. We evaluate the models' ability in a more rigorous way, and when only a few examples (e.g., $15$) are available for training. Unlike CLCCD works, we consider unseen languages as languages that are not seen during the training phase. We also study a combination of both, when both problem sets and languages are new to the model. Additionally, we apply our experiments for Ruby, in addition to well-studied languages, Java and C++. Finally, we apply few-shot learning algorithms and combine contrastive learning with the few-shot algorithm, which both are among the contributions of our work. 

% \textbf{Differences with the registered report:}

% \textcolor{purple}{In the registered report, we included Bert as a baseline model. However, as previous studies have not utilized this model for code clone detection and its performance was found to be suboptimal, it has been excluded from the present study. Additionally, we have used the contracode contrastive objective for both the base learner and the objective function of the meta-learner. Furthermore, instead of utilizing BigCloneBench and Poj-104 directly in our experiments, we used their schema to construct a new database utilizing CodeNET data. This was done to maintain consistency across all programming languages in our experiments.}


\section{Background}\label{sec:background}


\subsection{Few-Shot Learning}\label{sec: fewshot}

\begin{figure*}
    \centering
    \includegraphics[width=0.5\textwidth]{pictures/maml.png}
    \caption{This Figure, which is adopted from \cite{finn2017model}, shows the intuition behind the Model-Agnostic Meta Learning algorithm. Having a model that is parameterized with $\theta$ (A) cannot solve problems in the direction of $\theta^{*}_{1}$,  $\theta^{*}_{2}$, $\theta^{*}_{3}$ accurately. However, if the model is moved to point (B) through meta-learning, it can solve these problems using a few gradient steps.}
    \label{fig:maml}
\end{figure*} 

Few-shot learning is an area of machine learning where the model is trained using a restricted number of labeled data, sometimes as much as one sample in a downstream task. In this regard, few-shot learning algorithms and models learn a meta learner so that the meta learner can compare the labeled samples, which are called support set, with query examples, for which the model should predict the related class \cite{song2022comprehensive}. 
Figure \ref{fig:maml} shows the intuition behind Model-Agnostic Meta-Learning (MAML), the parametric-based algorithm used in this research for few-shot learning. 
In few-shot learning, we use three different datasets: \textit{train} set, \textit{support} set, and test set (also known as \textit{query} set). 
While the support set and test set share the same label space, the label space of the train set is disjoint with them. 
In this regard, if the support set consists of K samples per each unique class and there exist C classes in the support set, then this problem is called a K-shot C-way \cite{li2021concise}. 
It is possible to learn a classifier using only labeled samples in the support set. However, as the number of labeled data is scarce, the model would be overfitted to a few examples in the support set. Thus, few-shot learning algorithms learn a meta-learner capable of extracting transferable knowledge from the train set so that the model can be successfully fine-tuned using labeled data in the support set and performs more accurately on the test set \cite{li2021concise}.
Accordingly, to better train the meta-learner on the train set, an episode approach similar to \cite{vinyals2016matching} is utilized in most studies to mimic the few-shot learning setting for meta-learning. The process of training MAML is depicted in Figure \ref{fig:maml-train}. An episode is created in each training iteration by sampling C classes in the train set. Then, K-samples are chosen randomly for each class to serve as the support set.
Moreover, a query set is formed using the remaining samples. The model is then trained using the support set in each episode, and the losses for each episode (task) are computed using the query set to perform learning in the inner loop of MAML. Then, in the outer loop of MAML, The model parameters are updated using gradient descent on the aggregate loss computed over all tasks in the episode. The objective is to obtain a model that can quickly adapt to new tasks.
We follow this episode-based approach for code clone detection. 
 The details of how the algorithm is used in our study for few-shot learning are provided in Section \ref{subsec:maml}.



\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{pictures/MAML-Training.png}
    \caption{This Figure depicts the process of training in MAML. In MAML, an episode of various tasks is selected randomly in each iteration. Each episode simulates the C-way K-shot learning. This Figure depicts two-way 1-shot episodes. Then, MAML proceeds in two stages. In the inner loop, a base learner is used to compute a loss that is a mid-point for all the tasks in each episode using stochastic gradient steps. Then, a $\nabla L$ is computed using all losses in the inner loop. Finally, an outer loop performs a step of stochastic gradient descent over $\nabla L$. }
    \label{fig:maml-train}
\end{figure*} 


\subsection{Contrastive Learning}

\begin{figure*}
    \centering
    \includegraphics[width=0.85\textwidth]{pictures/contrastive.png}
    \caption{In this Figure, codes from the same problem set are considered positive samples. These positive instances can be from the same or different languages. Code snippets from other problem sets are considered negative examples. The contrastive objective aims to pull the representation of positive samples together and push the embedding of negative ones apart.}
    \label{fig:contrastive}
\end{figure*} 


Contrastive learning is a powerful self-supervised approach for unsupervised learning tasks, though it can be used for both supervised and unsupervised learning tasks. This method enables models to learn the representations without needing annotated data. 
In contrastive learning, instead of training a model to predict a ground truth label, the model aims to produce a representation that is similar for positive samples and is different from the negative pairs \cite{le2020contrastive}.
Accordingly, a strategy to generate positive and negative samples to learn the contrastive learning objective should be employed. For instance, ContraCode is a contrastive code representation learning model trained on a dataset of JavaScript code fragments. It utilizes a compiler-to-compiler translator to generate multiple variations of the same code as positive samples. In this way, other code snippets with different variations are considered negative examples in comparison to a given code \cite{jain-etal-2021-contrastive}. 
 In a contrastive supervised learning approach, on the other hand, the objective is defined such that the samples that belong to the same class have similar embeddings. Accordingly, positive samples belong to the same label space, and negative samples have different classes. %In this research, ContraCode is proposed to serve as the base learner of MAML, an unsupervised learning method. 
Figure \ref{fig:contrastive} shows how the contrastive objective is trained to build an embedding that is similar for positive examples and different for negative ones. 




%%%%%%%%%%%%%from RR%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> removed_Tables.tex <==
\begin{table}[]
    \centering
    \caption{The results of CodeBERT, RoBERTa and TBCCD in a 10-shot learning setup for unseen problems (JAVA)}
    \resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{@{}lccc@{}}\toprule
   Experiment& CodeBERT & RoBERTa & TBCCD\\
    \midrule

        Test for problems 16-30 & 48.1  & 46.4 & 49.5\\
        Test for problems 31-45
        & 50.4 & 47.9 & 51.3\\
        Test for problems 46-60
        &46.9 & 43.6 & 49.1
        \\
        Test for problems 61-75
        &49.4 & 47.8 & 51.3
        \\
        Test for problems 76-90
        & 47.6 & 47.1 & 49.2
        \\
        Test for problems 91-105
        & 51.2 & 50.6 & 51.8
        \\

    \bottomrule
   Mean & 48.93 & 47.2 & 50.36
   
    \end{tabular}}
    
    \label{tab:rq1-java-15shot}
\end{table}

\begin{table}[]
    \centering
    \caption{The results of CodeBERT, RoBERTa and TBCCD in a 5-shot learning setup for unseen problems (JAVA)}
    \resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{@{}lccc@{}}\toprule
   Experiment& CodeBERT & RoBERTa & TBCCD\\
    \midrule

        Test for problems 16-30 
        &
        45.7  & 41.2 & 47.5\\
        Test for problems 31-45
        & 48.7 & 43.1 & 49.7\\
        Test for problems 46-60
        &44.6 & 40.9 & 46.4
        \\
        Test for problems 61-75
        &48.1 & 43.9 & 49.3
        \\
        Test for problems 76-90
        & 45.9 & 45.2 & 50.4
        \\
        Test for problems 91-105
        & 49.8 & 47.3 & 50.1
        \\

    \bottomrule
   Mean & 47.13 & 43.6 & 48.9
   
    \end{tabular}}
    
    \label{tab:rq1-java-5shot}
\end{table}


\begin{table}[]
    \centering
    \caption{The results of MAML with different base learners (RUBY)}
    \resizebox{0.8\columnwidth}{!}{%
    \begin{tabular}{@{}lcccc@{}}\toprule
   Experiment& CodeBERT & RoBERTa & TBCCD & ContraCode
   \\
    \midrule

        Test for problems 16-30 &
        51.7 & 45.3 & 48.1 & 42.6\\
        Test for problems 31-45
        & 47.2 & 40.5 & 46.6 & 43.4\\ 
        Test for problems 46-60
        &51.2 & 39.2 & 45.2 & 39.8
        \\
        Test for problems 61-75
        & 45.6 & 43.7 & 41.8& 41.1
        \\
        Test for problems 76-90
        & 49.9 & 37.1 & 48.6 & 41.5
        \\
        Test for problems 91-105
        & 47.1 & 41.6 & 44.8 & 40.2
        \\

    \bottomrule
    Mean & 48.78 & 41.2 & 45.85 & 41.36
    \end{tabular}}
    
    \label{tab:mamal-problems-ruby}
\end{table}
